Circumvention by design -- dark patterns in cookie consents for online news outlets

To ensure that users of online services understand what data are collected and how they are used in algorithmic decision-making, the European Union's General Data Protection Regulation (GDPR) specifies informed consent as a minimal requirement. For online news outlets consent is commonly elicited through interface design elements in the form of a pop-up. We have manually analyzed 300 data collection consent notices from news outlets that are built to ensure compliance with GDPR. The analysis uncovered a variety of strategies or dark patterns that circumvent the intent of GDPR by design. We further study the presence and variety of these dark patterns in these "cookie consents" and use our observations to specify the concept of dark pattern in the context of consent elicitation.

==> GDPR Paper ArXiv (1)/CodingSummary_Than.tex <==
\section{Coding Summary}
The authors independently used the 5 categories and descriptions of dark patterns used in {gray} paper to examine and note the presence of dark patterns in all of our 300 sites. Each site is examined by two persons independently. The occurrences of dark patterns in the sites we have examined are summarized in the figure {add ref}. Some websites has changed their cookie popup designs and we have noted that whenever it happens {add the number}. 


%% conversations from the emails when doing the coding
Marija 
I wonder if we can propose a new list of dark patterns, specific for collecting consent? 
My list would be (in no particular order)

1. using on/off  sliders that are unlabelled with words so the user cannot tell for sure which colour means what 
2. the non-accept “option" is a link to a page where no actions are possible, for example there is only a description on how to change browser settings. 
3. the non-accept “option" link in the  text that is not emphasised (emphasised text is different colour or underlined)
4. using non contrasting colours for the consent panel together with "continue to use is acceptance”
5. different widgets for the accept and the not accept options 
6. using "non negative" words for the not-accept option
7. top right "x" that closes the panel (no information whether that counts as consent). 
8. consent panel obscures the text that describes what cookies do.

Our goal could be to define dark patterns in content collection so that they can be automatically detected. Currently dark pattern definitions require that the person recognises  intention, which is difficult to automatically detect. The motivation for these new specific dark patterns would be to enable automated detection of they exist, making it easier for authorities to detect violations, but also for companies to check compliance. Of course this would be a “whack-a-mole” game and it is a question if it is strictly better. 

Maybe if there is time we can check correlation between region that the webpage serves and dark pattern type. I noticed a lot of forced action and using is acceptance in non-eu pages. 

Frode 
I realized I never answered this very fine email from Marija. 

Yes I do think this is a very nice path. If we identify them like this, it is a good contribution. it also stands more out from the CHI paper. 
Is it easy to re-count the data from the comments we have made to see which of these patterns are most prevalent etc. ? 

I also think that if you look at the descriptions provided in the categorization- we have more and more precise descriptions of what kind of interface elements that were used. 

what are the relation between the patterns below and the dark patterns we used for categorizing?  

As for impact. I think just identifying these and - as oda suggested, provide an example/ template for how to give you a real choice would be more than enough
